TexFusion: Synthesizing 3D Textures with Text-Guided Image Diffusion Models

We present TexFusion (Texture Diffusion), a new method to synthesize textures for given 3D geometries, using large-scale text-guided image diffusion models. In contrast to recent works that leverage 2D text-to-image diffusion models to distill 3D objects using a slow and fragile optimization process, TexFusion introduces a new 3D-consistent generation technique specifically designed for texture synthesis that employs regular diffusion model sampling on different 2D rendered views. Specifically, we leverage latent diffusion models, apply the diffusion model's denoiser on a set of 2D renders of the 3D object, and aggregate the different denoising predictions on a shared latent texture map. Final output RGB textures are produced by optimizing an intermediate neural color field on the decodings of 2D renders of the latent texture. We thoroughly validate TexFusion and show that we can efficiently generate diverse, high quality and globally coherent textures. We achieve state-of-the-art text-guided texture synthesis performance using only image diffusion models, while avoiding the pitfalls of previous distillation-based methods. The text-conditioning offers detailed control and we also do not rely on any ground truth 3D textures for training. This makes our method versatile and applicable to a broad range of geometry and texture types. We hope that TexFusion will advance AI-based texturing of 3D assets for applications in virtual reality, game design, simulation, and more.

==> figures/multiview.tex <==
\begin{figure}[h]
    \centering
    \setlength{\tabcolsep}{0pt}
    \vspace{-0.15cm}
    \includegraphics[width=0.6\linewidth,trim=0 0 0 0,clip]{figures/inconsistency/multiview.png}
    \caption{Independently sampling SD2 w/depth produce disparate images in different views.}
    \label{fig:multiview}
    \vspace{-0.4cm}
\end{figure}

==> figures/sd_result.tex <==
\begin{figure}[H]

    \centering
    \vspace{-0.15cm}
    \setlength{\tabcolsep}{1pt}
    {\small 
    \renewcommand{\arraystretch}{0.8}
    \begin{tabular}{c c c}
    
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_160_brown rabbit_2_crop_0.png} &
         \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_160_brown rabbit_2_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_160_brown rabbit_2_crop_3.png} & \\
        \multicolumn{3}{c}{``brown rabbit"}\\
        
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_blonde girl with green eyes, hair in tied a bun, DSLR portrait photo_2_crop_0.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_blonde girl with green eyes, hair in tied a bun, DSLR portrait photo_2_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_blonde girl with green eyes, hair in tied a bun, DSLR portrait photo_2_crop_3.png} \\
        \multicolumn{3}{c}{``blonde girl with green eyes, hair in a tied } \\
        \multicolumn{3}{c}{bun, DSLR portrait photo"}  \\

        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_camper bag, camouflage_2_crop_0.png} &
         \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_camper bag, camouflage_2_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_camper bag, camouflage_2_crop_3.png} & \\
        \multicolumn{3}{c}{``camper bag, camouflage"}\\

        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_crocodile skin handbag_1_crop_0.png} &
         \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_crocodile skin handbag_1_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_crocodile skin handbag_1_crop_3.png} & \\
        \multicolumn{3}{c}{``crocodile skin handbag"}\\

    \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_medieval celtic House, stone bricks, wooden roof_1_crop_1.png} &
    \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_medieval celtic House, stone bricks, wooden roof_1_crop_2.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_medieval celtic House, stone bricks, wooden roof_1_crop_4.png} & \\
        \multicolumn{3}{c}{``medieval celtic House, stone bricks, wooden roof"}\\
        
           \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_old and rusty volkswagon beetle_0_crop_0.png} &
    \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_old and rusty volkswagon beetle_0_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_old and rusty volkswagon beetle_0_crop_3.png} & \\
        \multicolumn{3}{c}{``old and rusty Volkswagen beetle"}\\
 
        
        % \multicolumn{3}{c}{bun, anime illustration, portrait"} & \multicolumn{3}{c}{science fiction"} \\
        
    \end{tabular}}
    
    \caption{TexFusion + DDIM. 
    }
    \label{fig:even_more_results2}
\end{figure} 

==> figures/sd_result_single.tex <==
\begin{figure}[t]

    \centering
    \vspace{-0.15cm}
    \setlength{\tabcolsep}{1pt}
    {\small 
    \renewcommand{\arraystretch}{0.8}
    \begin{tabular}{c c c}
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_160_brown rabbit_2_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_blonde girl with green eyes, hair in tied a bun, DSLR portrait photo_2_crop_1.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_camper bag, camouflage_2_crop_1.png} \\
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_192_crocodile skin handbag_1_crop_0.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_medieval celtic House, stone bricks, wooden roof_1_crop_2.png} &
        \includegraphics[width=0.3\linewidth]{figures/sd2/sd2_rendered_nerf_256_old and rusty volkswagon beetle_0_crop_1.png} \\
    
        
        % \multicolumn{3}{c}{bun, anime illustration, portrait"} & \multicolumn{3}{c}{science fiction"} \\
        
    \end{tabular}}
    
    \caption{\small TexFusion + fully implicit DDIM sampling ($\sigma_{t_i}=0$). This setting emphasizes textural details, such as the leather (bottom, left), roof shingles (bottom, center), and rust (bottom, right).
    }
    \label{fig:even_more_results2}
\end{figure} 

==> section/method_old.tex <==

\section{Background}
\label{sec:Background}

\paragraph{Diffusion Models}~\cite{sohl2015deep,ho2020ddpm,song2020score} model a data distribution $p_{\text{data}}(\rvx)$ via \emph{iterative denoising} and are trained with \textit{denoising score matching}~\cite{hyvarinen2005scorematching,lyu2009scorematching,vincent2011,sohl2015deep,ho2020ddpm,song2020score}: Given samples $\rvx\sim p_{\text{data}}$, \emph{diffused} inputs $\rvx_t = \sqrt{\alpha_t} \rvx + \sqrt{1-\alpha_t} \boldsymbol{\epsilon}, \; \boldsymbol{\epsilon} \sim \gN(\mathbf{0}, \mI)$ are constructed; $\alpha_{t}$ defines a \emph{noise schedule}, parameterized via 
a diffusion-time $t$ (the presented formulation corresponds to a \emph{variance-preserving} schedule~\cite{song2020score}).
% , such that the logarithmic signal-to-noise ratio $\lambda_t = \log(\alpha_{t}^2/\sigma_t^2)$ monotonically decreases. 
A denoiser model $\boldsymbol{\epsilon}_\theta$ (parameterized with learnable parameters $\theta$) receives the diffused $\rvx_t$ as input and is
optimized minimizing the denoising score matching objective\looseness=-1
\begin{align}
\E_{\rvx \sim p_{\text{data}}, t \sim p_{t}, \boldsymbol{\epsilon} \sim \gN(\mathbf{0}, \mI)} \left[\Vert \boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\rvx_t; \rvc, t) \Vert_2^2 \right],
\label{eq:diffusionobjective}
\end{align}
where $\rvc$ is optional conditioning information, such as a text prompt. The model effectively learns to predict the noise $\boldsymbol{\epsilon}$ that was used to perturb the data (other formulations are possible~\cite{salimans2022progressive,karras2022elucidating}).
Furthermore, $p_t$ is a uniform distribution over the diffusion time $t$. 
The forward diffusion as well as the reverse generation process in diffusion models can be described 
% via stochastic differential equations 
in a continuous-time framework~\cite{song2020score}, but in practice a fixed discretization can be used~\cite{ho2020ddpm}.
The maximum diffusion time is generally chosen such that the input data is entirely perturbed into Gaussian random noise and an iterative generative denoising process 
% that employs the learned denoiser $\rvf_\theta$ 
can be initialized from such Gaussian noise to synthesize novel data.
% We use $p_t\sim\mathcal{U}\{0,1000\}$ and rely on a \emph{variance-preserving} noise schedule~\cite{song2020score}, for which $\sigma_t^2 = 1 - \alpha_t^2$ (Supp. Material for details). 

Classifier-free guidance~\cite{ho2021classifierfree} can be used for improved conditioning. By randomly dropping out the conditioning $\rvc$ during training, we can learn both a conditional and an unconditional model at the same time, and their predictions can be combined to achieve a stronger conditioning.



% Motivation on Diffusion model, notation for LDM, and notation for the rendering equations. 

% \paragraph{Image diffusion models.} are great.

% Inpainting via replacement is a thing (repaint)
% \begin{equation}
%     \vx_{t-1} = m \odot \vx_{t-1}^{\text{known}} + (1-m) \odot \vx_{t-1}^{\text{unknown}} \label{eqn:repaint}
% \end{equation}
We perform iterative diffusion model sampling via the \textit{Denoising Diffusion Implicit Models (DDIM)} scheme~\cite{song2021denoising}:
\begin{equation}
\begin{split}
    \vx_{i-1} = \sqrt{\alpha_{i-1}}\left(\frac{\vx_i - \sqrt{1 - \alpha_i} \boldsymbol{\epsilon}_\theta^{(t_i)}(\vx_i)}{\sqrt{\alpha_i}}\right) \\
    + \sqrt{1 - \alpha_{i-1} - \sigma_{t_i}^2} \cdot \boldsymbol{\epsilon}_\theta^{({t_i})}(\vx_i) + \sigma_{t_i} \boldsymbol{\epsilon}_{t_i}
\end{split}\label{eqn:ddim}
\end{equation}
with $\boldsymbol{\epsilon}_{t_i}\sim\gN(\mathbf{0}, \mI)$ and $\sigma_{t_i}$ is a variance hyperparameter.
We express obtaining $\vx_{i-1}$ via DDIM sampling as $\vx_{i-1} \sim \vf_\theta^{(t_i)}(\vx_{i-1} | \vx_i)$. See Supp. Material for more details.

\paragraph{Latent Diffusion Models (LDMs) and Stable Diffusion.} Instead of directly operating on pixels, LDMs~\cite{rombach2021highresolution} utilize an encoder $\mathcal{E}$ and a decoder $\mathcal{D}$ for translation between images $\xi$ and latents $\rvx\in X$ of a lower spatial dimension. The diffusion process is then defined over the distribution of $X$. \textit{Stable Diffusion} is an LDM trained on the LAION-5B image-text dataset. In addition to text-conditioning, \textit{Stable Diffusion 2.0} permits depth conditioning, where a depth map $D$ is appended 
% as a channel 
to $\rvx$. This allows detailed control of the shape and configuration of objects in its synthesized images.\looseness=-1

\paragraph{Rendering and Geometry Representation.} 
We generate textures on the surface of known input geometries.
In principle, our method applies to any geometry representation for which a textured surface can be rendered; in practice our experiments use a surface mesh $\mathcal{M} \subset \mathbb{R}^3$, with vertices $\mathcal{V} = \{v_i\},\ v_i \in \mathbb{R}^3$ and triangular faces $\mathcal{F} = \{f_i\}$ where each $f_i$ is a triplet of vertices. 
Textures are defined in 2D image-space in an injective UV parameterization of $\mathcal{M}$, $UV: p \in \mathcal{M} \mapsto (u,v) \in [0,1] ^ 2$, a common representation in computer graphics.
If needed, this parameterization can be automatically constructed via tools such as \textsc{xatlas}~\cite{theklaatlas2015,xatlas2016}.
We encode textures as multi-channel images discretized at pixels in UV space $\rvz \in \mathbb{R}^{(H \times W, C)}$, notationally collapsing the spatial dimension for simplicity.

We denote the rendering function as $\mathcal{R}(\rvz; \mathcal{M}, C): \rvz \mapsto \rvx $, $\rvx \in \mathbb{R}^{(h \times w, C)}$, which takes as input a mesh $\mathcal{M}$, camera $C$, and texture $\rvz$, and produces as output a rendered image.
The inverse of this function $\mathcal{R}^{-1}(\rvx; \mathcal{M}, C): \rvx \mapsto \rvz$ projects values from camera image-space onto the UV texture map. Notationally, we often omit the dependence on $\mathcal{M}$ and $C$ for brevity.
In this work, we do not model any lighting or shading effects, images are formed by directly projecting textures into screen space (and then decoding, for latent textures).\looseness=-1



%\section{Sequential Interlaced Multiview Sampler} 
\section{Texture Sampling with 2D Diffusion Models} 
\include{figures/overview_figure}

\input{figures/multiview}
Given a mesh geometry $\mathcal{M}$, a text prompt $y$, and a geometry (depth) conditioned image diffusion model $\theta$, how could one sample a complete surface texture? %Under the simplified rendering equations above, one can see that $\rvx$ is related to $\rvz$ via a permutation matrix: $\rvx = P \rvz$, where $P \in \{0,1\}^{(h\times w, H \times W)}$ and is orthogonal. \TIANSHI{This $x=Pz$ seems unnecessarily specific for this section, maybe just abstract to a rendering function R and and inverse rendering function IR, also don't really need to mention depth/text conditioning since these are not central to the SIMS story}
Assuming access to the rendering $\mathcal{R}$ and inverse rendering $\mathcal{R}^{-1}$ functions defined above, perhaps the most naive approach is to compute a set of $\{C_1, .., C_N\}$ camera views that envelopes the surface, render the depth map $d_n$ in each view, sample images from the image diffusion model with depth conditioning, and then back-project these images to the mesh surface %with average blending, i.e. $\rvz = \sum_{n=1}^N P_i^T \rvx_n / \sum_{n=1}^N P_n^T$, where $\rvx_n \sim p_\theta(\rvx|d_n, y)$. 
An obvious issue is that the image diffusion models in each view has no information about the generated result in other views, thus there is no coherency in the contents generated in each view (see Fig.~\ref{fig:multiview}). As an alternative, one may define a canonical order of camera views, and autoregressively condition image sampling in the subsequent views on previously sampled regions (as done in latent nerf? and TEXTure). However, for most geometries of interest (i.e. not a plane), a single (euclidean) projective camera can not observe the entirety of the geometry. Consequently, images synthesized early in the sequence could produce errors that are not reconcilable with the geometry that is observed later in the sequence (see Fig.~\ref{fig:inconsistency}). Thus, it is desirable for the image sampling distribution $p(\cdot|d_i, y)$ in each camera view to be conditioned on that of every other camera view.
\input{figures/inconsistency}
%The sequential nature of the denoising samping process allows us to symbiotically perform conditioning and synthesis.
\subsection{Interlaced sampling} Leveraging the sequential nature of the denoising process, we can interlace synchronization of content across views with the denoising steps within each view to achieve coherency over the entire shape. 
Suppose that at step $i$ of the denoising process, we have a set of partially denoised images $\{\rvx_{i, n}\}_{n=1}^N = \{\rvx_{i, 1} ... \rvx_{i, N}\}$. Our goal is to sample $\{\rvx_{i-1, n}\}_{n=1}^N = \rvx_{i-1, 1} ... \rvx_{i-1, N}$ that is 3D-consistent, i.e. two pixels in $\rvx_{i-1, a}, \rvx_{i-1, b}$ that project to the same point in 3D should have the same value. 
%$\{\rvx_{i-1, 1} ... \rvx_{i-1, N}\} \sim p_\theta(\rvx_{i-1, 1} ... \rvx_{i-1, N} | \rvx_{i, 1} ... \rvx_{i, N})$. Since we do not have a closed-form expresion for this distribution, we first make a simplifying assumption of independence in the same time step across views, thus we can write the joint as product of the marginals $p_\theta(\rvx_{i-1, 1} ... \rvx_{i-1, N} | \rvx_{i, 1} ... \rvx_{i, N}) = \prod_{n} p_\theta(\rvx_{i-1, n} | \rvx_{i, 1} ... \rvx_{i, N})$. Then, we approximate $p_\theta(\rvx_{i-1, n} | \rvx_{i, 1} ... \rvx_{i, N})$ by first aggregating $\{\rvx_{i, 1} ... \rvx_{i, N}\}$ into a latent texture map $\rvz_i$, rendering it in view $n$, and providing the rendered image as input to the diffusion model to approximate the distribution. 
Specifically, we aggregate the content from all views into a latent texture map by:
% \begin{equation}
%     \rvz_i = \frac{\sum_{n=1}^N P_i^T \rvx_{i, n}}{\sum_{n=1}^N P_n^T} \label{eqn:project_blend}
% \end{equation}
\begin{equation}
    \rvz_i = \frac{\sum_{n=1}^N \mathcal{R}^{-1}(\rvx_{i, n}; C_n)}{\sum_{n=1}^N \mathcal{R}^{-1}(\boldsymbol{I}; C_n)}, \label{eqn:project_blend}
\end{equation}
% \KK{The $\boldsymbol{I}$ isn't defined and the equation isn't entirely clear, I think. This is basically the same as MultiDiffusion, just written shorter, right?} where $\boldsymbol{I}$ is a unit vector with the same dimensionality as $\rvx_{i,n}$. Here, the denominator normalizes the value of each pixel by the number of cameras it is visible in.
We can then render $\rvz_i$, $\rvx_{i, n}' = \mathcal{R}(\rvz_i; C_n)$, for each $n$ to obtain $\{\rvx_{i, 1}' ... \rvx_{i, N}'\}$. Since they are rendered from one texture map, these images are 3D consistent by construction. Equation~\ref{eqn:ddim} can now be applied to each $\rvx_{i, n}'$ to draw a latent image at the next time step:
\begin{equation}
    \rvx_{i-1, n} \sim f_\theta^{(t_i)}(\rvx_{i-1, n}| \rvx_{i, n}' = \mathcal{R}(\rvz_i; C_n)). \label{eqn:parallel_sample}
\end{equation}
Then, $\{\rvx_{i-1, n}\}_{n=1}^N$ is used as the input for the next iteration. In essence, we've added a 3D consistency constraint to the diffusion trajectories such that pixels that need be consistent in multiple views are denoised in their average denoising direction over all views. % (i.e. pixels that map to the same location on the texture map). 
% Thus, we arrive at this expression for sampling $\{\rvx_{i-1, 1} ... \rvx_{i-1, N}\}$:
% \begin{equation}
%     \begin{split}
%         p_\theta( \{\rvx_{i-1, j}\}_{j=1}^N |  \{\rvx_{i, j}\}_{j=1}^N) \approx \prod_{n=1}^N p_\theta(\rvx_{i-1, n} | \rvx_{i, n}' = P_n \rvz_i(\{\rvx_{i, j}\}_{j=1}^N)) 
%     \end{split} \label{eqn:parallel_denoise}
% \end{equation}
While this approach prevent view-inconsistencies, averaging latents via Eqn.~\ref{eqn:project_blend} have unintended side-effects when diffusion models in different views predict denoising directions that are very inconsistent (in \cite{bar2023multidiffusion}, the case when $\min \mathcal{L}_{FTD}$ is large). As the average denoising direction does not follow any particular diffusion trajectory, one cannot guarantee that iterating through the diffusion process with the average prediction produce samples in the data distribution. 
To reduce inconsistency between predicted directions, one need to increase the overlap between each $\rvx_{i, n}$ such that the inputs to the diffusion model are similar from view to view. This would require a large number of cameras, and may even be unachievable in geometries with occlusions. Thus, we desire a method that can control $p_\theta(\{\rvx_{i-1, n}\}_{n=1}^N | \rvz_{i})$ such that its predictions are consistent.

% \KK{Your main RNDIR algorithm does not use interlaced sampling of 4.1, but only the sequential denoising and aggregation approach below, right? In that case, could we just push the whole 4.1 to the appendix in the interest of space and here just have a sentence ``We also explored abc, but it didn't work because def; see appendix.''. Saving some space and focusing on the most important things would be nice. The method section is long and complex already.}

\subsection{Sequential Denoising \& Aggregation} \label{sec:SDA}

One can observe that the $\rvx_{i-1, n}$s are not consistent because each $\rvx_{i-1, n}$ is sampled from the denoiser independently from other $\rvx_{i-1, m}, \, m \neq n$. Taking inspiration from the autoregressive modeling literature, we instead sample from an approximate the joint distribution via first decomposing it into a product of conditionals, and approximating each term in the product by using the diffusion model to denoise the renders of a dynamically updated latent texture map. Specifically, we decompose the joint distribution as follows (conditioning on depth and prompt omitted for space):
\begin{equation}
\begin{split}
    p_\theta( \{\rvx_{i-1, j}\}_{j=1}^N | \rvz_{i}) = p_\theta(\rvx_{i-1,1} | \rvz_{i}) \times \\
    \prod_{n=2}^N p_\theta(\rvx_{i-1, n} | \{\rvx_{i-1, j}\}_{j=1}^{n-1},  \rvz_{i}) \end{split}\label{eqn:seq_sampling}
\end{equation}
% \KK{Should it be $ \{\rvx_{i, j}\}_{j=1}^{n-1}$ in the set or $ \{\rvx_{i-1, j}\}_{j=1}^{n-1}$?}
We can see that the first term of the product is the same Eqn.~\ref{eqn:parallel_sample}, but the later terms depend on the outputs from previous views. We again model this dependency through the latent texture map. We first initialize $\rvz_{i-1, 0} = \rvz_{i}$ and obtain $\rvx_{i-1, 1}$ with Eqn.~\ref{eqn:parallel_sample}. 
Then, for each view starting at $n=1$, we inverse render $\rvx_{i-1, n}$ into texture space to obtain $\rvz_{i-1, n}' = \mathcal{R}^{-1}(\rvx_{i-1, n})$, and update the pixels of $\rvz_{i-1, n-1}$ that are newly visible in $\rvz_{i-1, n}'$ to obtain $\rvz_{i-1, n}$ (See Sec. \ref{sec:aggregating_latents} for details).
Then, in the in the $n+1$ iteration, since $\rvz_{i-1, n}$ contain regions at two noise scales (unseen regions are at noise scale $\sigma_i$, while visited regions are at noise scale $\sigma_{i-1}$), we add appropriate 3D consistent noise to the visited regions of $\rvz_{i-1, n}$ to match the noise scale of step $i$ before rendering it as input to $f_\theta$. Letting $M$ represent the mask for visited regions and $\epsilon_i \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$, we can write the sampling procedure for $\rvx_{i-1, n}$ as:
\begin{equation}
\begin{split}
    &\rvz_{i, n} = M \odot \left(\sqrt{\frac{\alpha_{i-1}}{\alpha_i}}  \rvz_{i-1, n-1} + \sigma_i \epsilon_i \right) + \left( \mathbf{1} - M\right) \odot \rvz_i \\
    &\rvx_{i-1, n} \sim f_\theta^{(t_i)}(\rvx_{i-1, n}| \rvx_{i, n}' = \mathcal{R}(\rvz_{i,n}; C_n))
\end{split}\label{eqn:SIMS}
\end{equation} 
% \TIANSHI{need to check coefficients}
By iteratively applying Eqn.~\ref{eqn:SIMS}, we obtain a sequence of 3D consistent images $\{\rvx_{i-1, n}\}_{n=1}^N$ and a texture map $\rvz_{i-1, n}$ that has been aggregated from these images. We can then decrement $i$ and repeat this process in the next time step. %\TIANSHI{Need an algorithm box here}

We name this approach Sequential Interlaced Multiview Sampler (SIMS). SIMS communicates the denoising direction of previous views to the current view, and resolves overlaps between views by the order of aggregation. Thereby it ameliorates the issue of inconsistent predictions while circumventing performance degradation due to the averaging of latent predictions during parallel aggregation. A complete algorithm box for SIMS can be found in the appendix. We also note that in the single-view case, SIMS is equivalent to standard DDIM sampling. 

% \TIANSHI{A paragraph comparing to closely related works here would make sense} 



%$ = P^T \rvx_{i-1, n} + ( 1 - P^T \boldsymbol{I}) \odot \rvz_{i-1, n-1}$ - that is, we update regions in $\rvz$ that are seen by camera $n$ after every step. 
% \KK{A pipeline figure would be very helpful. Also, the method section is overall long and complicated and needs to be shortened with more details going into appendix, I think.}

\section{The\ourmodel Algorithm} \KK{I am wondering whether it would make sense to merge sections 4 and 5 and have subsections for everything?} \TIANSHI{Anything specific to stable diffusion, our choice of renderer}
In section 4, we have presented a generic algorithm for sampling 3D consistent multi-view images and texture maps using 2D diffusion models. We now present an algorithm that uses SIMS to texture 3D meshes with depth-conditioned Stable Diffusion 2.0. As Stable Diffusion is a latent diffusion model, we apply SIMS in its latent space - $\rvx$ and $\rvz$ represent latent images and latent texture maps respectively. In this section, we address several challenges specific to using LDMs with SIMS, and detail our design choices to tackle these challenges.% such as using a neural color field for fusing decoded RGB images.
We find that a canonical set of cameras to work well for most objects, but cameras tailored to specific objects to improve resolution and ameliorate occlusion. We further illustrate a technique for obtaining high quality results by operating SIMS in a cascade of increasing resolutions.

\subsection{(Inverse) Rendering of Latent Textures}
We use \textsc{nvdiffrast} \cite{Laine2020diffrast} to efficiently render textured meshes via rasterization, as described in Section~\ref{sec:Background}.
Our implementation sets the rendered image size $h=w=64$ to match Stable Diffusion's UNet, with latent vectors of dimension $D=4$.
The texture image dimensions $H$ and $W$ are chosen based on the surface area of the mesh relative to its diameter. \NSHARP{what precise policy? (details can go in appendix)} 

For each non-background pixel $s$ in a rendered image $\rvx$, rasterization gives a corresponding location on the texture image via the UV map $(u,v) = UV(p)$, and we retrieve the value at the nearest texture pixel.
\NSHARP{``fetching'' a pixel is usually called \emph{texture sampling}, but that term is overloaded in this paper, so lets avoid it.}
This texture value is latent, and no shading or lighting is applied.
In other settings, texture data is often rendered with bilinear filtering and mip-maps to improve image quality and reduce aliasing, but in this setting we found it essential to \emph{avoid} such techniques. \NSHARP{could we show an example of this in the appendix?}
The issue is that when $t_i \ll 0$ early in the diffusion process, $\rvz_{i}$ and $\rvx_{i, \cdot}$ are dominated by noise, but interpolation and mip-mapping change the variance in the pixels $\rvx_{i, \cdot}$, thereby moving $\rvx_{i, \cdot}$ out of the training distribution of $\epsilon_\theta^{(t_i)}$.
Instead, we retrieve only nearest texture pixels for diffusion, and resolve aliasing and interpolation via a simple distillation post-process (Section~\ref{sec:distillation}).

Note that in this setting a rendered image is simply a selection of pixels from the texture maps, and thus we can leverage backpropagation to easily implement the inverse rendering function $\mathcal{R}^{-1}$.
Additionally, forward rasterization yields a depth map of the scene, which we use as a conditioning input to the diffusion model.

\input{figures/quality}

\subsection{Aggregating latent textures.}\label{sec:aggregating_latents} Recall from Sec.~\ref{sec:SDA}, before iterating through cameras $\{C_1, ..., C_N\}$, we first initialize $\rvz_{i-1, 0} = \rvz_{i}$ and $\rvx_{i, 1}' = \mathcal{R}(\rvz_{i-1, 0})$. Then, in each step, we obtain $\rvx_{i-1, n}$ from $f_\theta^{(t_i)}(\rvx_{i,n}')$, and inverse render it to get $\rvz_{i-1, n}' = \mathcal{R}^{-1}(\rvx_{i-1, n})$. Finally, we need to aggregate $\rvz_{i-1, n}'$ with $\rvz_{i-1, n-1}$ to obtain $\rvz_{i-1, n}$. We perform this aggregation step based on a simple heuristic that the value of each pixel $(u,v)$ in $\rvz$ should be determined by the camera that has the most ``direct and up-close" view to its corresponding point on the mesh. We measure view quality using image-space derivatives - the amount of change in UV coordinates per infinitesimal change in the image coordinate. This quantity is commonly used for determining mipmapping resolution and anti-aliasing, and it can be efficiently computed by nvdiffrast when rasterizing $\rvz_{i, n-1}$. For each pixel location $(p,q)$ in $\rvx_{i-1, n}$, we compute the negative jacobian magnitude as $-|\frac{\partial u}{\partial p} \cdot \frac{\partial v}{\partial q} - \frac{\partial u}{\partial q} \cdot \frac{\partial v}{\partial p}|$, and inverse render it to the texture space, which we denote as $Q_{i,n}$. Higher values of $Q_{i,n}(u,v)$ means that camera $n$ has a better view of $(u,v)$ (see Fig.~\ref{fig:quality}). %\KK{An example visualization of $Q_{i,n}$ would be nice, if possible, with some heatmap for quality.}. 
In addition, we compute $M_{i,n} = \mathcal{R}^{-1}(\boldsymbol{I})$, such that $M_{i,n}(u,v)$ represents the number of pixels in $\rvx_{i,n}'$ that received value from $\rvz_{i}(u,v)$. 

While iterating through cameras $1$ through $N$, we maintain mask $M_i$ (initialized to $0$), which is used to track which pixels of $\rvz_{i,n}$ has been seen by cameras up to $n$, and quality buffer $Q_i$ (initialized to $-\inf$), which is used to track the highest none-zero value of $Q_{i,n}$ at each $(u,v)$. The value at $(u,v)$ of $\rvz_{i-1, n}$ is determined as:
\begin{equation}
    \rvz_{i-1, n}(u,v) = \begin{cases}
        \frac{\rvz_{i-1, n}'(u,v)}{M_{i, n}(u, v)} &  \begin{split}M_{i, n}(u, v) > 0 \text{ , and} \\ Q_{i, n}(u,v) > Q_i(u,v)\end{split}\\
       % \rvz_{i-1, n-1}(u,v)                 &  M_{n}(u, v) > 0 \& (Q_{i, n}(u,v) < Q_i(u,v) || M_{i, n}(u, v) = 0) ,\\
        \rvz_{i-1, n-1}(u,v)                 & \text{otherwise.} \label{eqn:aggregation}
\end{cases}
\end{equation}
$M_{i}$ and $Q_i$ are then updated as: $M_i = \mathit{clamp}(M_{i, n} + M, 1)$ and $Q_i = \max{Q_{i,n}, Q_i}$.
We use Eqn.~\ref{eqn:aggregation} in conjunction with Eqn.\ref{eqn:SIMS} in SIMS to perform denoising of images in the sequence of camera views. 

We further note that a side effect of using nearest pixel filtering during texture sampling in SIMS is aliasing. 
When the image space derivative jacobian is much higher than 1 (low quality), neighboring pixels in screen space will have gaps when mapped to uv space. This results in incomplete filling of the latent texture map.
Conversely, when the  the image space derivative jacobian is much smaller than 1 (high quality), multiple screen space pixels $(p,q$ will map to the same $(u,v)$, creating uniform blocks in $\rvx$. Similar to interpolated latents, these blocks are particularly detrimental early during the diffusion process, as they cannot be correctly denoised by $\epsilon_\theta$ who is expecting high spatial variance.  Our quality-based aggregation overwrite low quality regions in the latent texture when higher quality views are available. Thus we can set the resolution of the texture map such that the image space derivatives in each view do not fall below $1$ (i.e. $\max Q_{i,n} < -1$) to prevent aliasing of the second type, and rely on cameras with better views to fix alising of the first type.

%the camera that views pixels in $\rvz$ that are viewed most dir
\subsection{From latent to RGB textures} 
\label{sec:distillation}
So far, we have described how to use SIMS to produce a set of 3D consistent latent images and latent texture maps, but have yet to describe how to translate this into a RGB texture map that can be rendered for viewing. Towards this, we experimented with multiple approaches and found performing multi-view distillation of decoded $\{\rvx_{0, n}\}_{n=1}^N$ with a neural color field to be most performant. 

Specifically, we use the decoder $\mathcal{D}$ of Stable Diffusion to decode $\{\rvx_{0, n}\}_{n=1}^N$ into $\{\xi_{n} = \mathcal{D}(\rvx_{0, n})\}_{n=1}^N$. Notably, decoding with $\mathcal{D}$ introduce inconsistencies such that $\{\xi_{n}\}_{n=1}^N$ is not 3D consistent even when $\{\rvx_{0, n}\}_{n=1}^N$ is 3D consistent \TIANSHI{image example here}. In stable Diffusion, each latent vector (pixel of $\rvx$) needs to carry the information of a $8 \times 8$ patch of RGB pixels. Thus, the value of the latent vector encode both color values and spatial patterns. We therefore cannot expect their decoded results to be equivariant to perspective transformations. 
To address this problem, we leverage a neural color field optimized with appearance based losses to smooth-out inconsistencies.
Since we know the ground-truth camera poses, we can directly obtain the 3D spatial coordinates $\{\mathit{xyz}_{n}\}_{n=1}^N$ of all pixels of $\{\xi_{n}\}_{n=1}^N$ by projecting pixels to the mesh surface. Background pixels that do not intersect any surface are discarded. Following \cite{magic3d}, we use a multi-resolution hash encoding based on instantNGP \cite{instantNGP} along with a shallow MLP $f_\phi$ to parameterize a function from 3D spatial coordinates to RGB values for each sample $\mathit{rgb} = f_\phi(\mathit{hash}(\mathit{xyz}))$. We then distill multi-view images $\{\xi_{n}\}_{n=1}^N$ in to this parametric function via optimization. 
Since our goal is to export $\phi$ into a texture map, we do not use any view dependent parameterization. To reconcile inconsistencies, we use both a standard $L2$ loss and a VGG-based perceptual loss, applied between $f_\phi$ and $\{\xi_{n}\}_{n=1}^N$, to train $\phi$. We use Adam with a learning rate of $0.01$, and optimization of $\phi$ converges within $100$ iterations. After optimization, we compute the spatial coordinate of the centers of each pixel in a high resolution texture map, and query $f_\phi$ to predict RGB values for the texture map. \TIANSHI{Refer to appendix section for more details}

\subsection{Geometry processing, camera, and multi-resolution refinement}
\KK{Some of these details that follow here can probably go into appendix.} \NSHARP{agreed.} We normalize $\mathcal{M}$ such that it fits inside a cube of side length 1, and center it at the origin. We align objects with meaningful ``front" to face the $+x$ direction, and ensure all objects are placed with $+y$ as ``up". Following \cite{dreamfusion}, we augment prompts with ``\{prompt\}, front/side/rear/top-view" based on the location of the camera; ``top-view" is used when the elevation of the camera is above $60^{\circ}$. 
We place cameras with perspective projection at a fixed distance of $1.5$ from the origin, and adjust the FOV to fit the object within the image. For most objects, we find that a set of nine cameras - all looking at the origin, eight spaced uniformly in surrounding the object (azimuth from $0^\circ$ to $315^\circ$ spaced $45^\circ$ apart, elevation of $30^\circ$), and one camera looking down the $-y$ direction - to work reasonable well for objects with reasonable aspect ratios and few occlusions. 

As the diffusion model relies on context captured in $\rvx$ to perform denoising, camera views that are too small w.r.t the size of the object often result in content drift - the texture in distant areas of the mesh can have conflicting content that are semantically inconsistent. This can be seen as our version of the Janus face problem known to Dreamfusion and similar approaches \cite{}. An obvious solution is to set the camera's FOV such that the entire object is visible in each view. However, this might not provide sufficient resolution for complex objects, since the texture resolution is upper-bounded by the resolution of the image diffusion model in each view (in the case of Stable Diffusion 2 with Depth, $512^2$). Our solution is to perform two rounds of RNDIR at different resolution scales to obtain higher resolution textures while retaining semantic consistency.

Specifically, We first run RNDIR using cameras that cover the entire object, and a low resolution latent texture map that is suitable for these cameras. We do not run view distillation in this first round as we are only interested in the latent texture map. We denote the denoised latent texture map from this step as $\rvz_{0, lr}$. We then use a second set of cameras with narrower field of view; these cameras are also more numerous to still cover the full object. We determine a new texture map resolution using the square of the ratio of the tangent of the old FOV over the new FOV - corresponding to the relative change in surface area covered by the camera before and after the change in FOV. We then up-sample $\rvz_{0, lr}$ with nearest neighbor filtering to this higher resolution, and stochastically encode it to a partially noised state (\eg $T=500$ in the DDPM time schedule). The second round of RNDIR uses these new cameras, and initializes SIMS with the partially noised latent texture map. The multi-view images produced by the second round of SIMS is used to produce the final output texture map via neural color field distillation. \KK{Out of curiosity: Could you also run the second refinement round with reconstruction guidance to reconstruct the low res version from the initial round (instead of the noise-denoise approach)? If I understand things correctly, it's more or less a form of superresolution, which can also be run with off-the-shelf diffusion models and reconstruction guidance.}

% A side effect of using nearest pixel filtering during texture sampling in SIMS is aliasing. 
% When the local uv space pixel density is higher than screen space pixel density, neighboring pixels in screen space will have gaps when mapped to uv space. This results in incomplete filling of the latent texture map.
% Conversely, when the local screen space pixel density is larger than the UV space pixel density, multiple screen space pixels $(p,q$ will map to the same $(u,v)$, creating uniform blocks in $\rvx$. Similar to interpolated latents, these blocks are particularly detrimental early during the diffusion process, as they cannot be correctly denoised by $\epsilon_\theta$ who is expecting high spatial variance. To control aliasing, one would need to set the resolution of the texture map such that the ratio of screen space pixel density to uv space pixel density is close to one. 


% motivate with the multiview example - using standard 2D diffusion samplers to simultaneously sample multiple views result in incoherent results; diffusion trajectories are not aware of the result from other views;
% Samping 3D inputs requires "harmonizing" multiple trajectories such that their outputs agree in value in overlapping regions, and are semantically and contextually consistent in non-overlapping regions. 
%In this section, we first provide an overview of RNDIR, followed by design details of its core components. %RNDIR can be viewed as a generalization of standard image diffusion denoising samplers to sets of 3D-coherent multiview images, which are combined into a surface texture. Similar to standard denoising samplers, RNDIR iterates through a decreasing sequence of time steps. We start with a randomly initialized latent

% At its core, ReNDIR operates reverse-time diffusion trajectories in multiple views and maintains consistency across the contents of all trajectories by interlacing synchronization steps via a shared latent texture map. Before each denoising step, the latent texture map is rendered into multiview latent images and fed as input to the denoiser. The $t_{i-1}$ state predicted by the denoising step is then projected to the latent texture map. The updates from the trajectories are aggreated in sequentially to resolve conflicts in overlapping texels. The results of the multiview trajectories are 3D consistent by-design, and can be composed into a coherent surface texture.

% \subsection{RNDIR} \TIANSHI{just laying all of the details here for now, we'll need to summarize and re-write later anyways} To sample a texture for input geometry $\mathcal{M}$ and text prompt $\mathcal{T}$, a latent texture map $\rvz_S \sim \mathcal{N}(0, \boldsymbol{I})$, of size $(H, W, C)$ is initialized ($C = 4$ for stable diffusion). RNDIR then iterates through $\{T_S, ... T_1\}$, a decreasing sequence of diffusion timesteps of length $S$, to denoise $\rvz_S$ into $\rvz_1$. 
% RNDIR iterates through a sequence of $N$ perspective cameras $\{c_i, ..., c_N\}$ that cover the surface of $\mathcal{M}$. 
% The main insight is that the texture image is connected to the image space via rendering equations
% In each step from $\rvz_i$ to $\rvz_{i-1}$, mask $M_i = \boldsymbol{0}$, quality buffer $Q_i = \boldsymbol{0}$, forward noise $\rvv_i \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$ and backward noise $\nu_i \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$, all with the same spatial dimension as $\rvz$, are initialized prior to iterating over the cameras. The mask $M_i$ is used to track which texels of $\rvz_{i,n}$ has been seen by cameras up to $n$, and the quality buffer $Q_i$ is used to track how well each texel of $\rvz_{i,n}$ has been seen by previous cameras.


% For the first camera ($n=1$), we set $\rvz_{i,1} = \rvz_i$. For cameras after the first, we include information gained from the previous denoising steps by sampling $\rvz_{i, n}$ from $q(\rvz_{i, n}|\rvz_i, \rvz_{i-1, n-1})$ i.e. $\rvz_{i, n} = M \odot \left(\frac{\alpha_{i-1}}{\alpha_i}  \rvz_{i-1, n-1} + \rvv_i \right) + \left( \mathbf{1} - M\right) \odot \rvz_i$

% For each camera $C_n$, $\mathcal{M}$ is rendered via rasterization and textured with the latent texture map via UV-mapping to produce latent image $\rvx_{i, n}$, and depth-map $d_{i, n}$ is also obtained via rasterization and used as geometry conditioning to the diffusion model. 
% \TIANSHI{To be continued...}
% % The previous state of the latent image is predicted as follows \cite{DDIM}:
% % \begin{align}
% %     \rvx_{i-1, n} &= \sqrt{\alpha_{i-1}}\left ( \frac{\rvx_{i, n} - \sqrt{1 - \alpha_i} \epsilon^{(t_i)}_\theta (\rvx_{i, n}; d_{i, n})}{\sqrt{\alpha_i}}\right) \\
% %     &- \sqrt{1 - \alpha_{i-1} - \sigma^2_i} \cdot \epsilon^{(t_i)}_\theta  (\rvx_{i, n}; d_{i, n}) 
% % \end{align}
% % In contrast to equation 12 of \cite{DDIM}, we do not add noise $\sigma_i \eps_i$ at 

% \TIANSHI{Then split method into parts, what key components do we want to highlight?}

% key novel idea is multiview synchronization - two benefits over inpainting: 1. dynamically correct view-incoherences in the sampling process (first view incoherences are impossible to correct in TEXTure) 2. invariance to order of views, doesn't need a canonical view
% - subpoints to this: 1. sequential aggregation and masking by uvda 2. forward-backward diffusion to correct for noise level, 3. x0 prediction is used as output, but xt is maintained, 4. uses DDIM for denoising

% second thing is the communication medium and data representation - whether texture map or implicit (depending on which works better experimentally), can highlight as a novelty too if implicit works better,
% - subparts - emphasize latent representation, rendering function, projection function, if using implicit, mention we can easily port to UV maps for interporability.

% third component - how to fight aliasing, need to preserve spatial variance prevents filtering at the forward rendering pass.

% last component - probably go into experimental details, post optimization with SDS loss, time clipping, text emphasis conditioning, dynamic thresholding, 
 
% alternative idea: what if we only connect views through the x0-prediction term in DDIM? $x_{t-1}^n = f(x_t^n) + h(x_0^\text{not} n)$. Basically views interact through a replacement guidance like term, and doesn't share a 3D consistent latent state. the x0 predictions can pass through the dec-rerender-enc stack to filter for 3D consistency. Perhaps sprinkle in this step with the lock step?


%While interpolating filters (such as bilinear, or mip-mapped textures) are more commonly used in graphics pipelines, we use nearest pixel filtering to exactly preserve the value of each pixel. This is particularly important during the earlier steps of the diffusion process 

% Under this simplified texturing process, $\rvx$ is related to $\rvz$ via a permutation matrix: $\rvx = P \rvz$, where $P \in \{0,1\}^{(h\times w, H \times W)}$ is an orthogonal permutation matrix that depends on $\mathcal{M}$ and $C$. Due to the high dimensionality of $P$, instead of forming it explicitly, we use the above-described pipeline for the forward rendering process, and backpropagate through it for the inverse rendering process.\KK{Is this permutation explanation relevant? The explanation before it seems fine and more intuitive.}

==> tables/user_study.tex <==
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l c c c} 
\toprule
Method & Quality & Semantic consistency & Coherency \\
\midrule
Magic3D        & 1         & $\textbf{1}$         & 1 \\
TEXTure    & 1          & 1     &  1\\
$\textbf{RNDIR}$ & $\textbf{1}$ & 1  & 1 \\
\bottomrule
\end{tabular}
\caption{User study
}
\vspace{-0.1cm}
\label{tb:user_study}
\end{table}
